Dominator Coloring and CD Coloring in Almost Cluster Graphs

In this paper, we study two popular variants of Graph Coloring -- Dominator Coloring and CD Coloring. In both problems, we are given a graph $G$ and a natural number $\ell$ as input and the goal is to properly color the vertices with at most $\ell$ colors with specific constraints. In Dominator Coloring, we require for each $v \in V(G)$, a color $c$ such that $v$ dominates all vertices colored $c$. In CD Coloring, we require for each color $c$, a $v \in V(G)$ which dominates all vertices colored $c$. These problems, defined due to their applications in social and genetic networks, have been studied extensively in the last 15 years. While it is known that both problems are fixed-parameter tractable (FPT) when parameterized by $(t,\ell)$ where $t$ is the treewidth of $G$, we consider strictly structural parameterizations which naturally arise out of the problems' applications. We prove that Dominator Coloring is FPT when parameterized by the size of a graph's cluster vertex deletion (CVD) set and that CD Coloring is FPT parameterized by CVD set size plus the number of remaining cliques. En route, we design a simpler and faster FPT algorithms when the problems are parameterized by the size of a graph's twin cover, a special CVD set. When the parameter is the size of a graph's clique modulator, we design a randomized single-exponential time algorithm for the problems. These algorithms use an inclusion-exclusion based polynomial sieving technique and add to the growing number of applications using this powerful algebraic technique.

==> dom_col_twin.tex <==
% !TEX root = dcoloring.tex

\section{\DomCol Parameterized by Twin Cover Size}
Consider a graph $G$. A subset $M$ of $V(G)$ is a \textit{Twin Cover} if for all $(u,v) \in E(G)$ either (i) $u \in M$ or $v \in M$ \textbf{or} (ii) $\closedneighbour{G}{u} = \closedneighbour{G}{v}$. This parameter was introduced by Ganian in 2015 \cite{Ganian2015} and has been used extensively in the world of parameterized complexity since. In this section, we will focus on the \DCMOD problem where $\family = \textsc{Cluster}$ and $M$ is a twin cover of the input graph. We denote this restriction of \DCMOD by \DCTC. Let $\DCTCinstance$ denote an instance of \DCTC. We let $\Q = \{Q_i\}^q_{i=1}$ denote the components of the cluster graph $G - M$ in such an instance and $V_{\Q}$ denote its vertices. The goal of this section is to prove the following theorem.

\begin{theorem}\label{DCTC is FPT}
	\DCTC is \fpt. There exists an algorithm that solves \DCTC in $\ordernoinput{2^{\order{k \log{k}}}}$-time.
\end{theorem}
In the subsection that follows, we design a general construct that, we believe, will be helpful in proving the (in)tractability of \DC parameterized by other structural parameters. We use this construct in \Cref{DC-TC} to prove \Cref{DCTC is FPT}.

%%%%%%%%%%%%%%%%%%%%%  Preliminaries   %%%%%%%%%%%%%%%%%%%%%
\input{preliminaries}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{\DCTC is  Fixed-Parameter Tractable}\label{DC-TC}

To prove \Cref{DCTC is FPT} we must construct (by \Cref{FPT collection of domcols}) for each instance $\I = \DCTCinstance$ of \DCTC, a collection of \pdc{}s $\Gamma(\I)$ which have properties listed in the lemma (replace $f(k)$ with $2^{\order{k \log{k}}}$). For this purpose, we require the following lemma due to Ganian~\cite{Ganian2015}. 
\begin{lemma} \label{Twin Cover Clique Neighbourhood}\cite{Ganian2015}
	Let $G$ be a graph. $M \subseteq V(G)$ is a twin cover of $G$ if, and only if, $G - M$ is a cluster graph and, if $\Q = \{Q_i\}^q_{i=1}$ are its connected components, for any $Q_i \in \Q$ and any $u,v \in V(Q_i)$, $\closedneighbour{G}{u} = \closedneighbour{G}{v}$.
\end{lemma}

By \Cref{Twin Cover Clique Neighbourhood}, every vertex of a clique $Q_i \in \Q$ has the same neighbourhood. With slight abuse of notation, in the rest of the section we use the term "the neighborhood of a clique" to mean the neighborhood of its vertices in $M$. Similarly, we say that a clique dominates a color class $c$ if each of its vertices dominates the color class $c$.


\begin{observation}\label{Twin Cover Clique Vertex Domination}
	Let $v \in Q_i$, for some $Q_i \in \Q$ be a vertex of $G$. Then, $v$ cannot dominate a color that has been used in both $M$ and $V(G) \setminus M$ in any \domcol of $G$.
\end{observation}
\begin{proof}
	Let $c$ be a color that has been used to color a $w \in M$ and $u \in V(G) \setminus M$. If $u \in Q_j$, where $i \neq j$, then, by Observation \Cref{Clique vertex domination}, $v$ cannot dominate $c$. Now, assume that $u \in Q_i$. Since a \domcol is a proper coloring of $G$, $w \notin \closedneighbour{G}{u}$. Since $M$ is a twin cover, $\closedneighbour{G}{u} = \closedneighbour{G}{v}$. Hence, $w \notin \closedneighbour{G}{v}$. Therefore, $v$ cannot dominate $c$. 
\end{proof}
\begin{corollary}\label{Twin Cover Unique Colors Required}
	Let $v \in Q_i$, for some $Q_i \in \Q$ be a vertex of $G$. If, in a \domcol $\rchi$ of $G$, if $v$ does not dominate any color that is used only to color vertices in $M$, then there exists a vertex $u \in Q_i$ which gets a color $c$ such that $|\rchi^{-1}(c)|=1$ .
\end{corollary}
%\begin{proof}
%	Let $C^{=0}_M$ denote the set of colors that are used only to color vertices in $M$ and $C^{>0}_M$ denote the set of colors that are used to color vertices in $M$ and $V(G) \setminus M$ by this \domcol of $G$.	Let $v \in Q_i$ be a vertex that does not dominate any color of $C^{=0}_M$. By \Cref{Twin Cover Clique Vertex Domination}, $v$ cannot dominate any color of $C^{>0}_M$. Moreover, by \Cref{Clique vertex domination}, $v$ cannot dominate a color used in some other clique. Hence, the color it dominates must be used only within the clique $Q_i$. Therefore, there exists a $u \in Q_i$ which gets a unique color.
%\end{proof}



Define $C_i=\{c_1,c_2\cdots c_i\}$. Observe that without loss of generality, we can assume that in any proper dominator coloring  the vertices in $M$ are colored using a subset of colors $C_k=\{c_1,c_2\cdots c_k\}$ and the vertices of $M$ dominates a color from the set of colors $C_{2k}$. For any arbitrary proper coloring $\rchi_M \colon M\mapsto C_k$ of $M$ and any arbitrary subset $C^\M\subseteq C_k$, let us define $M_D(\rchi_M, C^\M)\subseteq M$ as follows. Let $\Q_a$ be the set of cliques that dominate a color class in $C^\M$ and $\Q_b = \Q \setminus \Q_a$.  Let $M_a \subseteq M$ be the set of vertices which dominate a color class in $C^\M$. and let $M_b\subseteq M\setminus M_a$ be the set of vertices which neighbor one of the cliques in $\Q_b$. Define $M_D(\rchi_M, C^\M)=M\setminus (M_a\cup M_b)$. Consider the triplet $<\rchi_M, C^\M,\delta_0>$, where $\rchi_M \colon M\mapsto C_k$ is an arbitrary coloring of $M$, $C^\M\subseteq C_k$ is an arbitrary set of colors and $\delta_0\colon M_D(\rchi_M, C^\M)\mapsto C_{2k}$ is  an arbitrary function. For every choice of $<\rchi_M, C^\M,\delta_0>$ we define a \pdc $\pdci(\rchi_M, C^\M,\delta_0)$, as follows. 

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.63\textwidth]{fig_twin1}
	\caption{Illustration of construction of $\Gamma(\rchi_M,C^0,\delta_0)$.}
	\label{fig:twin1}
\end{figure}

For any vertex $v\in V[G]$, if $v$ dominates any color $c\in C^\M$, define $\delta(v)=c$. If a vertex dominates more than one color from  $ C^\M$, we choose an arbitrary color. 
Let $\Q_a$ be the set of cliques that dominate a color class in $C^\M$ and $\Q_b = \Q \setminus \Q_a$.  Without loss in generality, assume that $\Q_b=\{Q_1,Q_2\cdots,Q_{b'}\}$. We arbitrarily color one vertex from $Q_i \in \Q_b$ with color $c_{2k+i}$ (see \Cref{fig:twin1}). Denote the set of vertices colored by $V_{\Q}^1$ and the set of colors used by $C_{\Q}^1$.

Let $M_a \subseteq M$ be the set of vertices which dominate a color class in $C^\M$. For all $v\in M_a$, set $\delta(v)$ to be a color $c_i\in C^\M$ that $v$ dominates. Let $M_b\subseteq M\setminus M_a$ be the set of vertices which neighbor one of the cliques in $\Q_b$. Set, for $v\in M_b$, $\delta(v)=c_{2k+i}$, for an arbitrary $Q_i\in \Q_b$ that neighbors $v$. Let $M_c=M\setminus (M_a\cup M_b)$.

Observe every vertex $v$ except those in $M_D(\rchi_M, C^\M)$, dominates at least one color in the \pdc defined so far.
For any vertex $v\in M_D(\rchi_M, C^\M)$ we let $\delta(v)=\delta_0(v)$. 

%We define $M(\rchi_M,C^0)=M_c$ and for any vertex $v\in M_c$ we let $\delta(v)=\delta_0(v)$. 
If, for some $v\in M_D(\rchi_M, C^\M)$ where $\delta(v)=c_i$,  $v$ does not dominate $c_i$, then set $\pdci(\rchi_M, C^\M,\delta_0)=\emptyset$. Let $C_D = \{c  \mid \delta_0^{-1}(c)=\emptyset\}$ and $M_\emptyset$ be the set of vertices in $M$ that dominates a color class in $C_D$. Without loss in generality, assume that $C_D=\{c_{k+1},c_{k+2}\cdots c_{k+x}\}$. In order to ensure that the colors in $C_D$ is used at least once we do the following. Construct a bipartite graph $B_D$ with bipartition $(V_{\Q}, C_D)$ where $(v,c_i) \in E(B_D)$ if, and only if, $v\in \cap_{u\in \delta^{-1}(c_i)}\closedneighbour{G}{u}$. Refer to \Cref{fig:twin2} for a pictorial representation of the construction of $B_D$. If there does not exist a matching saturating $C_D$ in this graph, set $\pdci(\rchi_M, C^\M,\delta_0)=\emptyset$. Otherwise, select an arbitrary matching saturating $C_D$ and use $c_i \in C_D$  to color the vertex that it is matched to. Let the set of matched vertices from the cluster be $V_{\Q}^2$. 
Define $S=M\cup V_{\Q}^1 \cup V_{\Q}^2$

Consider the \pdc $\pdci(\rchi_M, C^\M,\delta_0)$.
%Let $\pdci$ be the partial coloring of $G$ that we have and $S$ be its domain. Observe that $\pdci$ is a \pdc of $G$. Set %$\Gamma(\rchi_M,C^0,\delta_0)=\{\pdci\}$. 
For any $\I = \DCTCinstance$ of \DCTC We let $\Gamma(\I)$ be the union of all $\pdci(\rchi_M, C^\M,\delta_0)$. Note that $|\Gamma(\I)| \in 2^{\order{k \log{k}}}$ and that it can be constructed in $\ordernoinput{2^{\order{k \log{k}}}}$-time.
\begin{figure}[ht]
	\centering
	\includegraphics[width=0.5\textwidth]{fig_twin2}
	\caption{Illustration of construction of $\Gamma(\rchi_M,C^0,\delta_0)$.}
	\label{fig:twin2}
\end{figure}


\begin{lemma}
	Any $\I = \DCTCinstance$ of \DCTC is a \yes instance iff there exist a \pdc $\pdci(\rchi_M,C^\M,\delta_0)\neq \emptyset\in \Gamma(\I)$ which can be extented to a proper \domcol.\label{lemma:domcolext}
\end{lemma}

\begin{proof}
	Consider an arbitrary instance $\I = \DCTCinstance$ of \DCTC. Observe that if there exist a \pdc $\Gamma(\rchi_M,C^\M,\delta_0)\in \Gamma(\I)$ which can be extended to a proper \domcol then it immediately follows that  $\I$ is a \yes instance. Let us assume that $\I$ is a \yes instance and $\rchi$ be the corresponding \domcol. WLG we can assume that there exists a $\pdci(\rchi_M,C^\M,\delta_0)\in \Gamma(\I)$, which agrees with $\rchi$ in $\rchi_M$, $C^\M$ and $\delta_0$ upto renaming of colors (follows from \Cref{Equivalence Class Assignment}). 
	
	Next, we construct a \domcol $\rchi'$ from $\rchi$ such that $\rchi'$ is an extension of $\pdci$ and uses at most $\ell$ colors. For a $Q\in \Q$, let $C_Q$ be the colors assigned to $Q$ by $\rchi$ and $\overline{C_Q}$ be the colors used in $\pdci$ in $Q$. For each $Q \in \Q$, we can use the colors in $C_Q\setminus \overline{C_Q}$ to color the rest of the vertices of $Q$. Since $\rchi$ is a \domcol of $G$ and agrees with $\pdci$ on $M$ while sharing the same domination function with it, it follows that this new coloring, which we call $\rchi'$, will also be a proper \domcol with domination function $\delta$. Moreover, it is clear that $|\rchi'| \leq |\rchi| \leq \ell$ and that $\rchi'$ is an extension of $\pdci$. This proves our claim. 
\end{proof}

By \Cref{FPT collection of domcols} and \Cref{lemma:domcolext}, we have the proof of \Cref{DCTC is FPT}.



==> preliminaries.tex <==
% !TEX root = dcoloring.tex
\subsection{Relating \DomCol and \ListCol} \label{Prelims}
%\begin{itemize}
%	\item Graph theoretic definitions. Induced subgraph, $G[V(G) \setminus M] = G - M$.
%	\item \fpt definitions. $\ordernoinput{\ }$.
%\end{itemize}

A \textit{partial coloring} $\widetilde{\rchi} \colon S \mapsto \widetilde{C}$ on $S \subseteq V(G)$ of a graph $G$ is a proper coloring of $G[S]$. 
 We now introduce the notion of a \pdc of a graph. 
\begin{mydefinition}
	A \textit{\pdc} is a triplet $(S,\widetilde{\rchi},\delta)$ where $S \subseteq V(G)$, $\delta \colon V(G) \mapsto \widetilde{C}$, and $\widetilde{\rchi} \colon S \mapsto \widetilde{C}$ is a partial coloring on $S$ such that for all $v \in V(G)$, $v$ dominates the color class $\delta(v) \in \widetilde{C}$. 
\end{mydefinition}
	

%We define a \textit{\pdc} as a triplet $(S,\widetilde{\rchi},\delta)$ where $S \subseteq V(G)$, $\delta \colon V(G) \mapsto \widetilde{C}$, and $\widetilde{\rchi} \colon S \mapsto \widetilde{C}$ is a partial coloring on $S$ such that for all $v \in V(G)$, $v$ dominates the color class $\delta(v) \in \widetilde{C}$. 

Throughout the section, we denote such a \pdc by $\pdci$. A \domcol $\rchi_d$ of $G$ is an \textit{extension} of a partial \domcol $\pdci$, if $\rchi_d$ agrees with $\pdci$ on $S$, and for all $v\in V(G)$,  $v$ dominates $\delta(v)$ with respect to $\rchi_d$. Analogous to the well-studied \PreCol problem (first introduced in \cite{Biro1992}), where we must decide if there exists a coloring of size $\ell$ which is an extension of a given partial coloring, we define \DCMODEXT.

\defparproblem{\DCMODEXT}
{A graph $G$, a set of vertices $M$ of cardinality $k$ such that $G - M \in \family$, and a partial \domcol $\pdci$ such that $M\subseteq S$; an integer $\ell$}
{$k$}
{Does there exist a  \domcol $\rchi_d$ of $G$ which is an extension of a partial \domcol $\pdci$ and $|\rchi_d|\leq \ell$?}

Another well known problem related to \Col is \ListCol which is defined as follows, for more information on the (parameterized) complexity of \ListCol, we refer the reader to \cite{Banik2020,Fiala2011,Gutin2021} and the references therein.
\defproblem{\ListCol\cite{Banik2020}}{A graph $G=(V,E)$ and a list $L$ of $|V|$ many set of colors with $L(v)$ being the entry for $v \in V$}
{Is there an assignment of colors $c:V \rightarrow \cup_{v\in V} L(v)$ such that it respects the lists $L$,  i.e. for any vertex $v$, $c(v)\in L(v)$ and for any two adjacent vertices $u$ and $v$, $c(v)\neq c(u)$?} 



%Let $\mathcal{P}(S)$, for any set $S$, denote the power set of $S$. Let $G$ be a graph and $C = \{c_1, c_2 \dots c_l\}$. In addition to these two input parameters, \ListCol has an additional parameter: a \textit{list function} $L \colon V(G) \mapsto \mathcal{P}(C)$ and asks the following question - does there exist a proper coloring $\rchi$ of $G$ such that $\rchi(v) \in L(v)$ for all $v \in V(G)$?  
 

Consider an instance $\DCMODEXTinstance$ of \DCMODEXT and let $H = G-M \in \family$. Moreover, assume that \ListCol can be solved in polynomial time when restricted to $\family$. We can carefully choose a list function $L$ on $V(H)$ so that a proper coloring of $H$ which respects $L$ can be used to color $V(G) \setminus S \subseteq V(H)$ and the coloring so obtained is an extension of $\pdomcolinstance$. The detailed construction of $L$ is given below as part of the proof of the theorem.
\begin{restatable}{theorem}{listcoleasyimpliesextiseasy}\label{ListCol is easy => Ext is easy}
	For any graph class $\family$ for which \ListCol is polynomial time solvable, \DCMODEXT is polynomial time solvable.
\end{restatable}
\begin{proof}
	Let $\family$ be a graph class for which \ListCol is polynomial time solvable. Let $\DCMODEXTinstance$ be an instance of \DCMODEXT. Then, $H = G-M \in \family$. If $C =\{c_1,c_2 \dots c_{\ell}\}$ is the total set of colors then, without loss in generality, we can assume that  $C_{\delta}\{c_1,c_2 \dots c_{\kappa}\}$ (for some $\kappa \leq \ell$) is the range of $\pdci$. 
	
	
	We now create a \ListCol instance $\ListColinstance$ by defining the list function $L$. For all $v \in V(H) \cap S$, we define $L(v) = \{\pdci(v)\}$. 
	For a color $c \in C_{\delta}$, let $V_\delta(c)$ be the set of vertices that dominate the color $c$ with respect to $\delta$, i.e. $V_\delta(c)=\delta^{-1}(c)$. Define $\closedneighbour{G}{V_\delta(c)}=\cap_{v\in V_\delta(c)} \closedneighbour{G}{v}$. 
	Observe that $\closedneighbour{G}{V_\delta^c}$ is exactly the set of vertices with the following property -- if any subset of vertices in $\closedneighbour{G}{V_\delta^c}$ is colored with $c$ then all the vertices in $V_\delta^c$ will continue dominating the color class $c$. 
	For ease of notation, for a $c \notin \im{\delta}$, we let $\closedneighbour{G}{V_\delta(c)} = V(G)$.
	Let $C_\kappa^\ell= \{c_{\kappa+1}, c_{\kappa+2}\dots c_{\ell}\}$
	For all $v \in V(H) \setminus S$, $L(v)=C_\kappa^\ell\cup \{c|v\in \closedneighbour{G}{V_\delta(c)}\}$. Next claim follows derectly from construction.
		%For all $v \in V(H) \setminus S$ include the colors $\{c_{\kappa+1}, c_{\kappa+2}\dots c_{\ell}\}$ in $L(v)$. For any color $c\in \{c_1,c_2 \dots c_{\kappa}\}$ include $c$ in $L(v)$ for $v \in V(H) \setminus S$ if, and only if, $c \notin \rchi_d(\closedneighbour{G}{v})$ and $v\in \closedneighbour{G}{V_\delta^c}$.
	\begin{myclaim}
		$\ListColinstance$ is a \yes instance of \ListCol iff $\DCMODEXTinstance$ is a \yes instance of \DCMODEXT.
	\end{myclaim}
	This concludes the proof.
%	\begin{proof}
%		Since $\ListColinstance$ is a \yes instance, there exists a feasible list coloring ${\rchi_L}$ of $H$. 
%		We construct a coloring $\rchi_d$ of $G$ as follows:
%		\[
%		\rchi_d(v) = \begin{cases}
%			\pdci(v) & \text{if } v \in S \\
%			{\rchi_L}(v) & \text{if } v \in V(H)
%		\end{cases}
%		\]
%		
%		Note that, for all $v \in S \cap V(H)$, $\rchi_L(v) = \pdci(v)$ since $L(v) = \{\pdci(v)\}$. Hence, $\rchi_d$ is indeed well-defined. Moreover, $|\rchi_d| \leq l$. We prove that $\rchi_d$ is an extension of $\pdci$. Observe that $\rchi_d$ induces a proper coloring of $H$ and $S$. By construction, for $v\in V(H)\setminus S$, $c\notin L(v)$ if $c$  is used to color a vertex in $\closedneighbour{G}{v}$. Thus $\rchi_d$ is a proper coloring. Next we prove that any vertex $v$ dominates the color class $\delta(v)$ in  $\rchi_d$.  Observe by construction the color $c=\delta(v)$ is only present in the list corresponding to a vertex $u$ if, and only if, $u\in \closedneighbour{G}{V^{c}_{\delta}}$ where $\closedneighbour{G}{V^{c}_{\delta}} \subseteq \closedneighbour{G}{v}$. Therefore the claim holds.
%	\end{proof}
%	\begin{myclaim}
%		$\ListColinstance$ is a \yes instance of \ListCol if $\DCMODEXTinstance$ is a \yes instance of \DCMODEXT.
%	\end{myclaim}
%	\begin{proof}
%		Since $\DCMODEXTinstance$ is a \yes instance, there exists an extension $\rchi_d$ of $\pdci$ with $|\rchi_d| \leq \ell$. We prove that the restriction of $\rchi_d$ on $H$, which we call $\overline{\rchi_d}$, is a list coloring of $H$ which respects the list function $L$. Let $v \in V(H)$. Since $\rchi_d$ is a proper coloring of $G$, $\rchi_d(v)$ is not used to color any vertices in $\closedneighbour{G}{v}$. If $\overline{\rchi_d}(v) \in \im{\delta}$, then $v \in \closedneighbour{G}{V^{c}_{\delta}}$. Therefore, $\overline{\rchi_d}(v) \in L(v)$. On the other hand, if $\overline{\rchi_d}(v) \notin \im{\delta}$, $\overline{\rchi_d}(v) \in L(v)$ by definition. This proves that $\overline{\rchi_d}$ is a proper coloring of $H$ which respects the list function $L$ with $|\overline{\rchi_d}| \leq \ell$. Therefore, $\ListColinstance$ is a \yes instance of \ListCol.
%	\end{proof}
%	
%	By these two claims, we have that $\DCMODEXTinstance$ is a \yes instance of \DCMODEXT if, and only if, $\ListColinstance$ is a \yes instance of \ListCol. Since $H \in \family$, $\ListColinstance$, and hence $\DCMODEXTinstance$, can be solved in polynomial time.
\end{proof}

For a family $\family$ where \ListCol is polynomial time solvable, while \Cref{ListCol is easy => Ext is easy} implies that \DCMODEXT is in \polytime, no such assertion can be made about \DCMOD. Assume that we have a collection $\Gamma(\I)$ of partial dominator colorings for each instance $\I = \DCMODinstance$ with the following property: $\DCMODinstance$ is a \yes instance of \DCMOD if, and only if, there exists a $\pdci \in \Gamma(\I)$ such that $\DCMODEXTinstance$ is a \yes instance of \DCMODEXT. Moreover, assume that $|\Gamma(\I)| \leq f(k)$ for some computable function $f$ which only depends on $k$ and that this collection can be constructed in $\ordernoinput{f(k)}$-time. Since for each $\pdci \in \Gamma(\I)$ we can correctly decide if $\DCMODEXTinstance$ is \yes or \no in polynomial time (by \Cref{ListCol is easy => Ext is easy}), in $\ordernoinput{f(k)}$-time, we can decide correctly if $\DCMODinstance$ is \yes or \no. In other words, if we can construct such a collection of partial dominator colorings $\Gamma(\I)$ for each instance $\I$ of \DCMOD, then \DCMOD is \fpt. 
\begin{lemma} \label{FPT collection of domcols}
	Let $\family$ be a graph family for which \ListCol is polynomial time solvable. Moreover, assume that for each instance $\I=\DCMODinstance$ of \DCMOD, there exists a collection $\Gamma(\I)$, with $|\Gamma(\I)| \leq f(k)$ which can be constructed in $\ordernoinput{f(k)}$-time for some computable function $f$, of partial dominator colorings such that $\I$ is a \yes instance if, and only if, there exists a $\pdci \in \Gamma(\I)$ such that $\DCMODEXTinstance$ is a \yes instance of \DCMODEXT. Then, there exists an algorithm that runs in $\ordernoinput{f(k)}$-time to solve \DCMOD.
\end{lemma}
In this paper, we are concerned with $\family \subseteq \textsc{Cluster}$. Therefore, to use \Cref{FPT collection of domcols}, we must prove that \ListCol can be solved in polynomial time when restricted to \textsc{Cluster}. It is known that \ListCol can be solved in polynomial time when restricted to cliques \Cref{BanikJPR20} which implies the following lemma.
%Following result is due to 
%\begin{figure}[ht]
%	\centering
%	\includegraphics[width=0.75\textwidth]{clq_list_col.pdf}
%	\caption{Illustration of the construction of $H$. Here, $Q_i = \{v_1,v_2,v_3,v_4,v_5\}$ and the list of colors for each vertex is given in brackets next to their labels.}
%	\label{List Coloring Clique Figure}
%\end{figure}
\begin{restatable}{lemma}{ListClusterPoly} \label{lemma:ListClusterPoly}
	\ListCol, restricted to cluster graphs, is polynomial time solvable.
\end{restatable}
%\begin{proof}
%	Let $\ListColinstance$ be an instance of \ListCol where $H$ is a cluster graph and $\Q = \{Q_i\}^q_{i=1}$ are the connected components of $H$. Note that each $Q_i \in \Q$ is a clique. Let $C = \{c_1,c_2 \dots c_\ell\}$. We create a bipartite graph $B_i$ on $(C,Q_i)$ as follows: $(c,v) \in E(B_i)$ if, and only if, $c \in L(v)$. We return \yes if, and only if, there exists a matching saturating $Q_i$ in $B_i$ for all $i \in \{1,2 \dots q\}$. Refer to \Cref{List Coloring Clique Figure} for an illustration of this construction.
%	
%	If $\ListColinstance$ is a \yes instance, then, since each $Q_i \in \Q$ is a clique, a coloring that respects the list function $L$ and uses at most $\ell$-many colors induces a matching saturating $Q_i$ in $B_i$. Therefore, our procedure will report \yes. On the other hand, if our procedure returns a \yes, the coloring obtained by assigning the color that each vertex is matched to is clearly one which uses at most $l$-many colors and respects $L$. Thus, in $\order{n^3}$-time, we can solve \ListCol when restricted to cluster graphs.
%\end{proof}
 
As a warm up before its use in \Cref{DC-TC}, we  first prove that \DC can be solved in polytime when restricted to cluster graphs using \Cref{FPT collection of domcols}. Note that the proof of the above fact from first principles is not too difficult as well. In this regard, we require two small observations.

\begin{restatable}{observation}{eqclassassignment} \label{Equivalence Class Assignment}
	Let $\rchi_d$ be a \domcol of a graph $G$ and $x,y \in V(G)$ such that $\closedneighbour{G}{x} = \closedneighbour{G}{y}$. Consider $\overline{\rchi_d}$ which swaps the colors of $x$ and $y$ and agrees with $\rchi_d$ on all other values. Then, $\overline{\rchi_d}$ is a \domcol of $G$ with $|\rchi_d| = |\overline{\rchi_d}|$.
\end{restatable}
\begin{proof}
	Since $\pdci$ agrees with the proper coloring $\rchi_M$ on $M$, no two adjacent vertices in $M$ are colored with the same color by $\pdci$. Note that $\im{\pdci} \setminus \im{\rchi_M} = C_D \cup C^1_\Q$ and $\pdci$ uses these colors exactly once while coloring. Moreover, $\pdci$ does not use any color in $\im{\rchi_M}$ outside $M$. Thus, $\rchi_d$ is a partial coloring of $M$.  By construction, every vertex in $V(G)$ dominates the color class $\delta(v)$. Therefore, $\pdci$ is a \pdc of $G$.
\end{proof}

\begin{observation}\label{Clique vertex domination}
	Let $G$ be a cluster graph and $\Q = \{Q_i\}^q_{i=1}$ denote its connected components. Let $v \in V(Q_i)$ for some $Q_i \in \Q$. Then, $v$ cannot dominate a color class which is used to color a vertex $u \in V(Q_j)$ for some $i \neq j$ in any \domcol of $G$.
\end{observation}

\begin{lemma} \label{DC can be solved quickly in clusters}
	\DC, restricted to cluster graphs, is polynomial time solvable.
\end{lemma}
\begin{proof}
	Let $\I = \DCinstance$ be an instance of \DC where $G$ is a cluster graph. Let $\Gamma(\I) = \{\pdci\}$ where $\pdci$ is a partial \domcol obtained by uniquely coloring an arbitrary vertex in each clique and assigning this color as the one to dominate for all vertices in that clique. The correctness of this construction follows from \Cref{Equivalence Class Assignment,Clique vertex domination}. The lemma now follows from \Cref{lemma:ListClusterPoly} and \Cref{FPT collection of domcols}. 
\end{proof}


\begin{comment}
	
	\begin{itemize}
		\item Define $\partitionfn{\cdot}$.
		\item Its relation to Bell's number, cite the paper.
	\end{itemize}
	
	\begin{equation} \label{partition number}
		\partitionfn{s} = {\left( \frac{s}{\ln s} \right)}^s
	\end{equation}
	Structural parameterized version:
	
	
	A ``reduced" version:
	\defparproblem{\DCMODR}
	{A graph $G$, a set of vertices $M$ of cardinality $k$ such that $G - M \in \family$ and a partition $\P = \{P_1, P_2 \dots P_\kappa\}$ of $M$ such that $G[P_i]$ is an independent set for each $P_i \in \P$; an integer $l$}
	{$k$}
	{Does there exist a \domcol{} $\rchi_d$ of $G$ with $|\rchi_d|\leq l$ such that for any $u,v \in M$, $\rchi_d(u) = \rchi_d(v)$ iff $u,v \in P_i$ for some $P_i \in \P$?}
	\begin{lemma} \label{enough to solve reduced version}
		If we can solve \DCMODR in $f(n,k)$-time, for some function $f$, then we can solve \DCMODR in $\order{f(n,k) \cdot \partitionfn{k}}$-time.
	\end{lemma}
	\begin{proof}
		Assume that there exists an algorithm $\A$ which solves \DCMODR in $f(n,k)$-time. We construct an algorithm $\A'$ to solve \DCMOD as follows: for each partition $\P$ of $M$, $\A'$ calls $\A$ with parameters $\DCMODRinstance$ and reports \yes if at least one such instance is a true instance of \DCMODR and \no otherwise. Since $|M| = k$, there are $\order{\partitionfn{k}}$-many partitions of $M$. Hence, $\A'$ runs in $\order{f(n,k) \cdot \partitionfn{k}}$-time. 
		
		Consider an instance $\DCMODinstance$ of \DCMOD. If $\A'$ returns \yes for this instance, then there exists a partion $\P$ of $M$ such that $\DCMODRinstance$ is a true instance of \DCMODR. Hence, $\DCMODinstance$ is a true instance of \DCMOD. On the other hand, if $\DCMODinstance$ is a true instance of \DCMOD, then there must exist a partition $\P$ of $M$ such that $\DCMODRinstance$ is a true instance of \DCMODR. Hence, in this case $\A'$ would have returned \yes. 
		
		This proves that $\A'$ is an algorithm which runs in $\order{f(n,k) \cdot \partitionfn{k}}$-time and solves the \DCMOD problem.     
	\end{proof}
	\begin{lemma}
		\DC can be solved in polynomial time when restricted to cluster graphs.
	\end{lemma}
	\begin{proof}
		Let $\DCinstance$ be an instance of \DC where $G$ is a cluster graph.  Let $\Q = \{Q_i\}^q_{i=1}$ be the set of cliques that form $G$. Note that a vertex $v \in Q_i$, for some $Q_i \in \Q$, cannot dominate a color that has been used to color a vertex in $Q_j \in \Q$, where $i \neq j$. Therefore, in any \domcol of $G$, there must exist at least one color that is used only in each $Q_i \in \Q$. Since the $Q_i$s are cliques, every vertex in them must be assigned different colors. Hence, if $\rchi_d$ is a \domcol of $G$, 
		\[
		|\rchi_d| \geq q + \max^q_{i=1}|Q_i| -1
		\] 
		We prove that this lower bound is tight by constructing a \domcol of $G$ whose size meets this bound. For each $Q_i \in \Q$ assign an arbitrary vertex a unique color $c_i$. Now, in the largest-sized clique, color all the vertices with different colors (all of which are different from the unique colors $\{c_1, c_2 \dots c_q\}$). Reuse these colors to color the uncolored vertices of the rest of the cliques. Clearly, this is a \domcol of $G$ (a $v \in Q_i$ dominates the color class $c_i$) and uses ($q + \max^q_{i=1}|Q_i| -1$)-many colors. Therefore, this is \domcol is optimal.
		
		Given an instance $\DCinstance$ of \DC where $G$ is a cluster graph, we can compute $\Q = \{Q_i\}^q_{i=1}$ in quadratic time. We return \yes if $q + \max^q_{i=1}|Q_i| -1 \leq l$ and \no otherwise. The correctness of this algorithm follows from the arguments presented in the previous paragraph.
	\end{proof}
	\defproblem{\DCEXTN}
	{A graph $G$, a subset of vertices $M$, a partial \domcol $\pdci$ of $G$ which has colored all vertices in $M$ (and possibly other vertices as well), the set of colors, $C_{\old}$, used by $\pdci$, a subset $C_{\no}$ of $C_{\old}$, and a domination function $D \colon{} V(G) \mapsto C_{\old}$ with respect to $\pdci$; an integer $l$}
	{Does there exist an extension $\rchi_d$ of $\pdci$ with $|\rchi_d| \leq l$, which respects the domination function $D$, and does not use the colors in $C_{\no}$ outside of those vertices colored by $\pdci$?}
	\begin{lemma}\label{Constructing Optimal Extensions Lemma}
		If $\DCEXTNinstance$ is an instance of \DCEXTN such that $G - M$ is a cluster graph, then, this instance can be solved in polynomial time.
	\end{lemma}
	\begin{proof}
		We will show that we can construct an optimal extension of $\pdci$, and therefore decide if $\DCEXTNinstance$ is a \yes or a \no instance, in polynomial time.
		
		An optimal extension $\rchi_d$ of $\pdci$ must maximize the number of vertices that are colored using colors from $C_{\old}$ so as to minimize the number of new colors used. To ensure that $\rchi_d$ remains a proper coloring, we impose the following constraint: a color cannot be used to color two adjacent vertices. Moreover, since $\rchi_d$ respects the domination function $D$, a vertex $u$ uncolored by $\pdci$ can be colored by a $c \in \im{D}$ only if $u$ is adjacent to all the vertices which dominate $c$. Succinctly, $u$ can be colored with a $c \in \im{D}$ only if $u \in \cap_{v \in D^{-1}(c)}\openneighbour{G}{v}$. 
		
		
		\begin{algorithm}
			\caption{\DCEXTN where $G-M$ is a Cluster Graph}
			\label{Constructing Optimal Extensions}
			\SetAlgoLined
			\DontPrintSemicolon
			\KwIn{An instance $\DCEXTNinstance$ of \DCEXTN{} such that $G - M$ is a cluster graph}
			\KwResult{\yes if $\DCEXTNinstance$ is a \yes instance, \no otherwise}
			\For{$Q_i \in \Q$}
			{
				$E_i \longleftarrow \emptyset$\;
				$\widetilde{Q_i} \longleftarrow$ uncolored vertices of $Q_i$\;
				\For{$(c,u) \in (C_{\old} \setminus C_{\no})\times \widetilde{Q_i}$}
				{
					\If{$c$ is not used to color any vertex in $\openneighbour{G}{u}$}
					{
						\If{$c \in D(V)$}
						{
							\If{$u \in \cap_{v \in D^{-1}(c)}N_G(v)$}
							{
								$E_i \longleftarrow E_i \cup \{(c,u)\}$\;
							}
						}
						\Else
						{
							$E_i \longleftarrow E_i \cup \{(c,u)\}$\;
						}
					}
					
				}
				Consider the bipartite graph $B_i$ on $C_{\old} \setminus C_{\no}$ and $\widetilde{Q_i}$ with edge set $E_i$\;
				Find a maximum matching $M_i$ of $B_i$\;
				${unc}_i \longleftarrow |\widetilde{Q_i}| - |M_i|$\;
			}
			$unc \longleftarrow \max^q_{i=1} {unc}_i$\;
			\If{$|C_{\old}|+unc\leq l$}
			{
				\Return{\yes} \;
			}
			\Else
			{
				\Return{\no}\;
			}
		\end{algorithm}
		
		Let $\Q = \{Q_i\}^q_{i=1}$ be the set of cliques that form $G - M$ ($G - M$ is a cluster graph). Since $\pdci$ has already colored the vertices in $M$, the uncolored vertices are in one of the $Q_i$s. Let $\widetilde{Q_i}$ denote the set of uncolored vertices of $Q_i$. Note that no two vertices in $Q_i$, and hence in $\widetilde{Q_i}$, can be assigned the same color. Therefore, the problem of maximizing the number of old colors used to color the uncolored vertices can be thought of as finding a maximum matching on the bipartite graph $B_i$ on $C_{\old} \setminus C_{\no}$ and $\widetilde{Q_i}$ for each $Q_i \in \Q$ whose edges are defined by the constraints discussed in the previous paragraph. An vertex is colored to its matched color. Let $unc_i$ denote the number of uncolored vertices in $Q_i$ after this step and $i^* = \arg\max^q_{i=1} {unc}_i$ and $unc = unc_{i^*}$. Consider a set of new colors $C_{\new}$ containing $unc$-many colors. Complete the coloring of each $Q_i$ by assigning each of its uncolored vertices a different color from $C_{\new}$. Let $\rchi_d$ denote this coloring of $G$. \Cref{Constructing Optimal Extensions} presents the procedure discussed in this paragraph to construct $\rchi_d$. \Cref{Constructing Optimal Extensions} returns \yes if $\rchi_d$ uses at most $l$-many colors and \no otherwise.
		
		By construction, $\rchi_d$ is an extension of $\pdci$. We prove that it is indeed optimal. Assume that there exists an extension $\overline{\rchi_d}$ of $\pdci$ such that $|\overline{\rchi_d}| < |\rchi_d|$. Then, the total number of new colors used by $\overline{\rchi_d}$ is strictly less than those used by $\rchi_d$. Therefore, the  number of new colors used in $Q_{i^*}$ by $\overline{\rchi_d}$ is strictly less than $unc$. This implies that the number of old colors used  in $Q_{i^*}$ by $\rchi_d$ is strictly less than that used by $\overline{\rchi_d}$. This is impossible since \Cref{Constructing Optimal Extensions} maximizes the number of old colors assigned to $Q_{i^*}$ by finding a maximum matching between $C_{\old}$ and $\widetilde{Q_{i^*}}$. 
		
		Therefore, $\rchi_d$ is an optimal extension of $\pdci$. This proves the correctness of \Cref{Constructing Optimal Extensions}. Since the algorithm runs in polynomial time (in $\order{n^4}$-time), this completes the proof of the lemma. 
	\end{proof}
\end{comment}

